Galactic Radio Explorer: an all-sky monitor for bright radio bursts

We present the Galactic Radio Explorer (GReX), an all-sky monitor to probe the brightest bursts in the radio sky. Building on the success of STARE2, we will search for fast radio bursts (FRBs) emitted from Galactic magnetars as well as bursts from nearby galaxies. GReX will search down to ten microseconds time resolution, allowing us to find new super giant radio pulses from Milky Way pulsars and study their broadband emission. The proposed instrument will employ ultra-wide band (0.7-2 GHz) feeds coupled to a high performance (receiver temperature 10 K) low noise amplifier (LNA) originally developed for the DSA-110 and DSA-2000 projects. In GReX Phase I (GReX-I), unit systems will be deployed at Owens Valley Radio Observatory (OVRO) and Big Smoky Valley, Nevada. Phase II will expand the array, placing feeds in India, Australia, and elsewhere in order to build up to continuous coverage of nearly 4$\pi$ steradians and to increase our exposure to the Galactic plane. We model the local magnetar population to forecast for GReX, finding the improved sensitivity and increased exposure to the Galactic plane could lead to dozens of FRB-like bursts per year.

==> authors.tex <==
\author[Connor et al.]{%
L.~Connor$^{1, 2}$,
M.~C.~Miller$^{3}$,
D.~W.~Gardenier$^{2, 1}$ 
\\
~\\
%% ----------------- Institutes --------------- 
$^{1}$ Anton Pannekoek Institute, University of Amsterdam, Postbus 94249, 1090 GE Amsterdam, The Netherlands\\ 
$^{2}$ ASTRON, the Netherlands Institute for Radio Astronomy, Oude Hoogeveensedijk 4,7991 PD Dwingeloo, The Netherlands\\ 
$^{3}$Department of Astronomy and Joint Space-Science Institute, University of Maryland, College Park, MD 20742-2421
}


